Leave-One-Out Neighborhood Smoothing for Graphons: Berry--Esseen Bounds and Edge-Wise Confidence Intervals

We develop a framework for edge-wise inference in graphon-based random networks. The proposed leave-one-out neighborhood procedure excludes the target vertex when selecting neighbors, then averages the selected vertices' edges to that target. Conditional on the latent probabilities and selected neighborhood, these edges are independent. This structure yields finite-sample concentration inequalities and a Berry--Esseen bound for fluctuations about the selected-neighborhood mean. Under blockwise graphon regularity, quantitative two-hop identifiability, and across-block separation, we control the smoothing bias uniformly over latent positions, including positions near block boundaries. Together with an observable variance estimator, this gives Gaussian confidence intervals for individual edge probabilities with asymptotically correct pointwise coverage. We also establish finite-sample empirical Bernstein coverage for the selected-neighborhood mean, Gaussian inference under weaker bandwidth conditions on identical-profile blocks, and inference for target pairs chosen measurably from the latent positions. Finally, we derive an expected-risk identity for leave-one-out cross-validation at each fixed neighborhood size. Simulations assess interval coverage, variance estimation, and estimation error.

==> generated_results/regenerated_20260831/simulation_tables_regenerated.tex <==
\begin{table}[tb]
\centering
\caption{Rate experiment at
$h_n=\operatorname{round}(n^{2/3})$. ``Scaled'' denotes
$n^{2/3}$ times the LOO MSE.}
\label{tab:rate-simulation}
\begin{tabular}{lrrrrr}
\toprule
Model & $n$ & $h_n$ & LOO MSE & ZLZ MSE & Scaled \\
\midrule
Kink & 200 & 34 & 0.00779 & 0.00843 & 0.266 \\
Kink & 500 & 63 & 0.00438 & 0.00424 & 0.276 \\
Kink & 1000 & 100 & 0.00248 & 0.00268 & 0.248 \\
Kink & 2000 & 159 & 0.00169 & 0.00168 & 0.269 \\
\addlinespace
Linear & 200 & 34 & 0.00792 & 0.00803 & 0.271 \\
Linear & 500 & 63 & 0.00456 & 0.00474 & 0.288 \\
Linear & 1000 & 100 & 0.00286 & 0.00300 & 0.286 \\
Linear & 2000 & 159 & 0.00171 & 0.00170 & 0.271 \\
\addlinespace
SBM & 200 & 34 & 0.00661 & 0.00646 & 0.226 \\
SBM & 500 & 63 & 0.00337 & 0.00373 & 0.212 \\
SBM & 1000 & 100 & 0.00218 & 0.00228 & 0.218 \\
SBM & 2000 & 159 & 0.00125 & 0.00140 & 0.198 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Feasible Gaussian inference under
$h_n=\operatorname{round}(n^{3/5})$. Widths are truncated to $[0,1]$.
The column $\widehat V/V$ reports the Monte Carlo mean of $\widehat V_{ij}^{\mathrm{emp}}/V_{ij}$.
The ZLZ interval is a descriptive plug-in Gaussian comparator.}
\label{tab:gaussian-inference}
\begin{tabular}{lrrrrrr}
\toprule
Model & $n$ & $h_n$ & LOO cov. & ZLZ cov. & LOO width & $\widehat V/V$ \\
\midrule
Kink & 200 & 24 & 0.937 & 0.923 & 0.397 & 1.007 \\
Kink & 500 & 42 & 0.946 & 0.935 & 0.301 & 1.004 \\
Kink & 1000 & 63 & 0.932 & 0.930 & 0.245 & 1.002 \\
Kink & 2000 & 96 & 0.954 & 0.958 & 0.199 & 1.001 \\
\addlinespace
Linear & 200 & 24 & 0.945 & 0.925 & 0.396 & 1.010 \\
Linear & 500 & 42 & 0.935 & 0.929 & 0.299 & 1.002 \\
Linear & 1000 & 63 & 0.945 & 0.940 & 0.245 & 1.001 \\
Linear & 2000 & 96 & 0.958 & 0.975 & 0.199 & 1.004 \\
\addlinespace
SBM & 200 & 24 & 0.957 & 0.948 & 0.366 & 1.008 \\
SBM & 500 & 42 & 0.929 & 0.898 & 0.276 & 0.999 \\
SBM & 1000 & 63 & 0.938 & 0.932 & 0.226 & 0.998 \\
SBM & 2000 & 96 & 0.975 & 0.971 & 0.183 & 1.001 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Empirical Bernstein performance for the conditional
neighborhood mean under $h_n=\operatorname{round}(n^{3/5})$. ``Full'' is
the fraction of truncated intervals equal to $[0,1]$.}
\label{tab:bernstein-inference}
\begin{tabular}{lrrrrr}
\toprule
Model & $n$ & $h_n$ & EB cov. & EB width & Full \\
\midrule
Kink & 200 & 24 & 1.000 & 0.997 & 0.960 \\
Kink & 500 & 42 & 1.000 & 0.899 & 0.000 \\
Kink & 1000 & 63 & 1.000 & 0.699 & 0.000 \\
Kink & 2000 & 96 & 1.000 & 0.515 & 0.000 \\
\addlinespace
Linear & 200 & 24 & 1.000 & 0.997 & 0.958 \\
Linear & 500 & 42 & 1.000 & 0.891 & 0.000 \\
Linear & 1000 & 63 & 1.000 & 0.697 & 0.000 \\
Linear & 2000 & 96 & 1.000 & 0.515 & 0.000 \\
\addlinespace
SBM & 200 & 24 & 1.000 & 0.962 & 0.615 \\
SBM & 500 & 42 & 1.000 & 0.758 & 0.000 \\
SBM & 1000 & 63 & 1.000 & 0.627 & 0.000 \\
SBM & 2000 & 96 & 1.000 & 0.491 & 0.000 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Oscillatory stress test under the inference bandwidth.
The design is not used to validate the main theorem because quantitative
two-hop identifiability has not been verified. The column $\widehat V/V$ is the Monte Carlo mean of the empirical-to-oracle variance ratio.}
\label{tab:wiggly-stress}
\begin{tabular}{rrrrrrr}
\toprule
$n$ & $h_n$ & LOO cov. & ZLZ cov. & LOO width & $\widehat V/V$ & Std. bias \\
\midrule
200 & 24 & 0.878 & 0.885 & 0.373 & 1.034 & 0.472 \\
500 & 42 & 0.910 & 0.890 & 0.277 & 1.015 & 0.308 \\
1000 & 63 & 0.955 & 0.955 & 0.226 & 1.022 & 0.251 \\
2000 & 96 & 0.950 & 0.946 & 0.181 & 1.003 & 0.213 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Additional stress-test results at $n=500$.
Point-estimation MSEs use $h_n=63$ and Gaussian inference uses $h_n=42$. The column $\widehat V/V$ reports a Monte Carlo mean.}
\label{tab:additional-stress-tests}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrr}
\toprule
Model & LOO MSE & ZLZ MSE & LOO cov. & ZLZ cov. & LOO width & $\widehat V/V$ \\
\midrule
Sinusoidal & 0.00377 & 0.00379 & 0.948 & 0.935 & 0.286 & 1.001 \\
Additive linear & 0.00463 & 0.00470 & 0.935 & 0.925 & 0.294 & 0.996 \\
Spiky & 0.00249 & 0.00252 & 0.921 & 0.925 & 0.237 & 0.978 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tb]
\centering
\caption{Independent neighborhood-size sweep for the kink
graphon at $n=1000$. The final column is the Monte Carlo mean of
$|B_{ij}^{(-j)}|/\sqrt{V_{ij}}$.}
\label{tab:bandwidth-sweep}
\begin{tabular}{rrrr}
\toprule
$c$ & $h_n$ & LOO MSE & Mean standardized bias \\
\midrule
0.5 & 50 & 0.00519 & 0.166 \\
1.0 & 100 & 0.00278 & 0.231 \\
2.0 & 200 & 0.00149 & 0.320 \\
4.0 & 400 & 0.00075 & 0.436 \\
\bottomrule
\end{tabular}
\end{table}


==> generated_results/regenerated_20260831/tables/additional_stress.tex <==
\begin{table}[tb]
\centering
\caption{Additional stress-test results at $n=500$.
Point-estimation MSEs use $h_n=63$ and Gaussian inference uses $h_n=42$. The column $\widehat V/V$ reports a Monte Carlo mean.}
\label{tab:additional-stress-tests}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrr}
\toprule
Model & LOO MSE & ZLZ MSE & LOO cov. & ZLZ cov. & LOO width & $\widehat V/V$ \\
\midrule
Sinusoidal & 0.00377 & 0.00379 & 0.948 & 0.935 & 0.286 & 1.001 \\
Additive linear & 0.00463 & 0.00470 & 0.935 & 0.925 & 0.294 & 0.996 \\
Spiky & 0.00249 & 0.00252 & 0.921 & 0.925 & 0.237 & 0.978 \\
\bottomrule
\end{tabular}
\end{table}


==> generated_results/regenerated_20260831/tables/wiggly.tex <==
\begin{table}[tb]
\centering
\caption{Oscillatory stress test under the inference bandwidth.
The design is not used to validate the main theorem because quantitative
two-hop identifiability has not been verified. The column $\widehat V/V$ is the Monte Carlo mean of the empirical-to-oracle variance ratio.}
\label{tab:wiggly-stress}
\begin{tabular}{rrrrrrr}
\toprule
$n$ & $h_n$ & LOO cov. & ZLZ cov. & LOO width & $\widehat V/V$ & Std. bias \\
\midrule
200 & 24 & 0.878 & 0.885 & 0.373 & 1.034 & 0.472 \\
500 & 42 & 0.910 & 0.890 & 0.277 & 1.015 & 0.308 \\
1000 & 63 & 0.955 & 0.955 & 0.226 & 1.022 & 0.251 \\
2000 & 96 & 0.950 & 0.946 & 0.181 & 1.003 & 0.213 \\
\bottomrule
\end{tabular}
\end{table}

